Change of variable formul{\ae} for regularizing slowly decaying and oscillatory Cauchy and Hilbert transforms

Formul{\ae} are derived for expressing Cauchy and Hilbert transforms of a function $f$ in terms of Cauchy and Hilbert transforms of $f(x^r)$. When $r$ is an integer, this corresponds to evaluating the Cauchy transform of $f(x^r)$ at all choices of $z^{1/r}$. Related formu\ae\ for rational $r$ result in a reduction to a generalized Cauchy transform living on a Riemann surface, which in turn is reducible to the standard Cauchy transform. These formul{\ae} are used to regularize the behaviour of functions that are slowly decaying or oscillatory, in order to facilitate numerical computation and extend asymptotic results.

==> Slowly decaying Cauchy/osccommon.tex <==
\function{Gma}{\Gamma}

\defoperator{ii}{I}

\defoperator{QA}{Q^A}
\defoperator{QL}{Q^L}
\defoperator{QB}{Q^B}
\defoperator{QF}{Q^F}
%\defoperator{L}{{\cal L}}
\def\L{{\cal L}}
\def\P{{\cal P}}
\def\M{{\cal M}}
\defoperator{MA}{{\cal M}^\star}



\def\iif{\ii[f]}
\def\QAf{\QA[f]}
\def\QFf{\QF[f]}
\def\QLf{\QL[f]}
\def\QBf{\QB[f]}

\def\iig_#1[#2]{I_{#1}\br[{#2}]}
\defoperator{iigg}{I_g}
\def\iigf[#1]{\iigg[f,#1]}
\def\iigfo{\iigf[\Omega]}

\def\QAg_#1[#2]{Q^A_{#1}\br[{#2}]}
\defoperator{QAgg}{Q^A_g}
\def\QAgf[#1]{\QAgg[f,#1]}
\def\QAgfo{\QAgf[\Omega]}

\def\QLg_#1[#2]{Q^L_{#1}\br[{#2}]}
\defoperator{QLgg}{Q^L_g}
\def\QLgf[#1]{\QLgg[f,#1]}
\def\QLgfo{\QLgf[\Omega]}

\def\QBg_#1[#2]{Q^B_{#1}\br[{#2}]}
\defoperator{QBgg}{Q^B_g}
\def\QBgf[#1]{\QBgg[f,#1]}
\def\QBgfo{\QBgf[\Omega]}

\def\QFg_#1[#2]{Q^F_{#1}\br[{#2}]}
\defoperator{QFgg}{Q^F_g}
\def\QFgf[#1]{\QFgg[f,#1]}
\def\QFgfo{\QFgf[\Omega]}

\function{Lv}{\L[v]}

\def\sig_#1(#2){\sigma_{#1}\fpr(#2)}

\def\ew#1{\E^{\I \omega #1}}
\def\ewp(#1){\E^{\I \omega \pr({#1})}}
\def\ewg(#1){\E^{\I \omega g\pr(#1)}}
\def\ewgg{\E^{\I \omega g}}
\def\ewx{\E^{\I \omega x}}

\def\iw{\I \omega}

\def\nodes{\seq_1^\nu x}
\def\mults{\seq_1^\nu m}
\def\basis{\seq_1^n \psi}

\def\Dv{{\cal D}}
\def\Dm{\Dv^{\vc m}}
\def\Dek{\Dv^{\vc{e}_k}}

\def\qq{\vc q}


\def\vcnodes{\seq_1^\nu {\xx}}
\def\vcbasis{\seq_1^n \psiB}
\let\vcmults=\mults


\def\sjacobiandd_#1^#2{\vc{J}_{#1}^{#2}}
\def\sjacobiand_#1^#2{\sjacobiandd_{#1}^{#2}(\xx)}

\def\sjacobian_#1{\sjacobiand_{#1}^d}
\def\sjacobiantk{\sjacobian_{T_\ell}}


\def\oiw{{1 \over \I \omega}}



\def\fO(#1){\Oh\fpr({#1})}
\def\fOw#1{\fO(\omega^{#1})}
\def\Ow#1{\O(\omega^{#1})}

\def\Leq#1{\L[v](#1)=f(#1)}
\def\Leqp#1{\L[v]'(#1)=f'(#1)}
\def\Leqn#1{\Leq{x_#1}}
\def\Leqnp#1{\Leqp{x_#1}}
\def\Leqpn^#1#2{\L[v]^{(#1)}(#2)=f^{(#1)}(#2)}
\def\Leqnpn^#1#2{\Leqpn^{#1}{x_#2}}

\def\Leqv#1{\L[\vv](#1)=\ff(#1)}
\def\Leqvn#1{\Leqv{x_#1}}
  
\def\ds{\dkf{\vc{s}}}



\def\vv{\vc v}  
\def\xx{\vc x}  
\def\xV{\vc x}  
\def\mm{\vc m}
\def\cc{{\vc c}}
\def\bb{{\vc b}}
\def\ff{\vc f}
\def\FF{\vc F}
\def\yy{\vc y}
\def\ee{\vc e}
\def\dd{\vc d}


%%%%%%%%%%%%
% GMRES
%%%%%%%%%%%%

\def\Km_#1{{\cal K}_{#1}}
\defoperator{K}{{\cal K}_n}
\def\Kn{\K[{\cal L},f] }

\def\Schrodinger{Schr\"odinger}


%%%%%%%%%%%%%%
% RH


\def\RHp{RH problem}
\def\RHf{RH formulation}
\def\RHa{RH approach}



==> Slowly decaying Cauchy/socommon.tex <==
\def\pr(#1){\left({#1}\right)}
\def\br[#1]{\left[{#1}\right]}
\def\set#1{\left\{{#1}\right\}}
\def\ip<#1>{\left\langle{#1}\right\rangle}
\def\iip<#1>{\left\langle\!\langle{#1}\right\rangle\!\rangle}

\def\fpr(#1){\!\pr({#1})}

\def\floor#1{\left\lfloor#1\right\rfloor}
\def\ceil#1{\left\lceil#1\right\rceil}

%\def\function#1#2{\def#1(##1){#2\fpr({##1})}}
\def\function#1#2{\expandafter\def\csname #1\endcsname(##1){#2\fpr({##1})}
				\expandafter\def\csname #1p\endcsname(##1){#2'\fpr({##1})}
				\expandafter\def\csname #1pp\endcsname(##1){#2''\fpr({##1})}
				\expandafter\def\csname #1pn\endcsname##1(##2){#2^{\pr({##1})}\fpr({##2})}				}
\def\defoperator#1#2{\expandafter\def\csname #1\endcsname[##1]{#2\!\br[{##1}]}}

\def\ffunction#1{\function{#1}{#1}}

\def\O(#1){{\cal O}\!\left(#1\right)}

\def\Oo(#1){{\rm o}\!\left({#1}\right)}


\def\fO(#1){\Oh\fpr({#1})}

\def\mspan#1{{\rm span}\set{#1}}

\def\rdiag#1{{\rm rdiag}\,(#1)}
\def\Rdiag{{\rm rdiag}\,}

%
%	List of predefined functions
%


\def\dkfn^#1#2{\,{\rm d}^#1 #2}
\def\dkf#1{\,{\rm d}#1}

\def\I{{\rm i}}
\def\E{{\rm e}}

\def\H_#1^#2(#3){H_#1^{(#2)}\fpr({#3})}
\def\J_#1(#2){{\rm J}_#1\!\pr(#2)}
\def\cl{{\rm cl}\,}

\def\erfi{{\rm erfi}\,}

\def\half{{1 \over 2}}

\def\LL#1{L_#1}

\let\grad=\nabla
\let\lap=\Delta
\let\union=\bigcup

\def\ala{{\it \`a la\/}}
\def\apriori{{\it a priori\/}}
\def\apostiori{{\it a postiori\/}}


\def\fd#1{^{({#1})}}


\def\dx{\dkf{x}}
\def\dy{\dkf{y}}
\def\dz{\dkf{z}}
\def\dt{\dkf{t}}
\def\dV{\dkf{V}}
\def\ds{\dkf{\vc s}}

\def\ddxn^#1{{\dkf{}^#1 \over \dkfn^#1{x}}}

\def\ddx{{\dkf{} \over \dx}}
\def\pddx{{\partial \over \partial x}}
\def\pddy{{\partial \over \partial y}}

\def\pddxf#1{{\partial #1 \over \partial x}}
\def\pddyf#1{{\partial #1 \over \partial y}}

\def\Dv{{\cal D}}
\def\Dm{\Dv^{\vc m}}
\def\Dek{\Dv^{\vc{e}_k}}


\def\Bignorm#1{\Bigl\| #1 \Bigr\|}
\def\norm#1{\left\| #1 \right\|}
\def\Bignnnorm#1{ \Bigl | \mskip-1.5mu \Bigl\|\,{#1}\, \Bigr\|\mskip-1.5mu \Bigr |} 
\def\norminf#1{\norm{#1}_\infty}

\def\seq_#1^#2#3{\set{#3_{#1},\ldots,#3_{#2}}}
\def\infseq#1{\set{#1_{1},#1_{2},\ldots}}

\def\TT{\Bbb T}
\def\UU{\Bbb U}

\let\real=\R
\let\nonnegative=\N


\def\abs#1{\left|{#1}\right|}


\ffunction{f}
\ffunction{g}


%
%	Map a list using \mapfunction
%
% Usage:
% {\def \mapfunction#1{$#1^2$}
%
% \map a,b,c,d,\void.}


\def\mapengine#1,#2.{\mapfunction{#1}\ifx\void#2\else\mapengine #2.\fi }

\def\map[#1]{\mapengine #1,\void.}

\def\mapenginesep_#1#2,#3.{\mapfunction{#2}\ifx\void#3\else#1\mapengine #3.\fi }

\def\mapsep_#1[#2]{\mapenginesep_{#1}#2,\void.}

 \def\vczero{{\bf 0}}
 \def\vcone{{\bf 1}}
%\def\vcbr{\br}
\def\vcbr[#1]{\pr({#1})}


\def\bvect[#1,#2]{
{
\def\dots{\cdots}
\def\mapfunction##1{\ | \  ##1}
	\sopmatrix{
		 \,#1\map[#2]\,
	}
}
}

\def\vect[#1]{
{\def\dots{\ldots}
	\vcbr[{#1}]
}}

\def\vectt[#1]{
{\def\dots{\ldots}
	\vect[{#1}]^{\top}
}}

\def\Vectt[#1]{
{
\def\mapfunction##1{##1 \cr} 
\def\dots{\vdots}
	\sopmatrix{
		\map[#1]
	}
}}


\def\Notation#1{
\def\notationaddtab##1:##2={##1 & ##2\;& =}
\bigskip
\def\\{\cr\notationaddtab}
\halign{\quad\vtop{\parindent=0pt\hsize=0.33\hsize
						\strut##\strut}\hfil & \qquad \hfil $##$ & $##$ \hfil \cr\notationaddtab
	#1
}
\bigskip\noindent
}


\def\LHopital{L'Hopital's rule}

\def\qqquad{\qquad\quad}
\def\qqqquad{\qquad\qquad}

\def\qand{\quad\hbox{and}\quad}
\def\qqand{\qquad\hbox{and}\qquad}
\def\qfor{\quad\hbox{for}\quad}
\def\qqfor{\qquad\hbox{for}\qquad}
\def\qas{\quad\hbox{as}\quad}
\def\qqas{\qquad\hbox{as}\qquad}
\def\qqor{\qquad\hbox{or}\qquad}
\def\qqwhere{\qquad\hbox{where}\qquad}

\def\questionequals{= \!\!\!\!\!\!{\scriptstyle ? \atop }\,\,\,}
\def\simlimit_#1{\,\,\,\sim \!\!\!\!\!\!\!\!\!{ \atop \scriptscriptstyle #1 }}


\def\Xint#1{\mathchoice
   {\XXint\displaystyle\textstyle{#1}}%
   {\XXint\textstyle\scriptstyle{#1}}%
   {\XXint\scriptstyle\scriptscriptstyle{#1}}%
   {\XXint\scriptscriptstyle\scriptscriptstyle{#1}}%
   \!\int}
\def\XXint#1#2#3{{\setbox0=\hbox{$#1{#2#3}{\int}$}
     \vcenter{\hbox{$#2#3$}}\kern-.5\wd0}}
\def\ddashint{\Xint=}
\def\dashint{\Xint-}



\def\rad^#1#2{\,\,{}^#1\!\!\!\!\sqrt{#2}\,}




\def\Figuretwofixed#1#2#3\par{
\Figuretwow{#1}{#2}{0.48 \hsize}{#3}\par
}


\def\Painleve{Painlev\'e}


==> socommon.tex <==
\def\pr(#1){\left({#1}\right)}
\def\br[#1]{\left[{#1}\right]}
\def\set#1{\left\{{#1}\right\}}
\def\ip<#1>{\left\langle{#1}\right\rangle}
\def\iip<#1>{\left\langle\!\langle{#1}\right\rangle\!\rangle}

\def\fpr(#1){\!\pr({#1})}

\def\floor#1{\left\lfloor#1\right\rfloor}
\def\ceil#1{\left\lceil#1\right\rceil}

%\def\function#1#2{\def#1(##1){#2\fpr({##1})}}
\def\function#1#2{\expandafter\def\csname #1\endcsname(##1){#2\fpr({##1})}
				\expandafter\def\csname #1p\endcsname(##1){#2'\fpr({##1})}
				\expandafter\def\csname #1pp\endcsname(##1){#2''\fpr({##1})}
				\expandafter\def\csname #1pn\endcsname##1(##2){#2^{\pr({##1})}\fpr({##2})}				}
\def\defoperator#1#2{\expandafter\def\csname #1\endcsname[##1]{#2\!\br[{##1}]}}

\def\ffunction#1{\function{#1}{#1}}

\def\O(#1){{\cal O}\!\left(#1\right)}

\def\Oo(#1){{\rm o}\!\left({#1}\right)}


\def\fO(#1){\Oh\fpr({#1})}

\def\mspan#1{{\rm span}\set{#1}}

\def\rdiag#1{{\rm rdiag}\,(#1)}
\def\Rdiag{{\rm rdiag}\,}

%
%	List of predefined functions
%


\def\dkfn^#1#2{\,{\rm d}^#1 #2}
\def\dkf#1{\,{\rm d}#1}

\def\I{{\rm i}}
\def\E{{\rm e}}

\def\H_#1^#2(#3){H_#1^{(#2)}\fpr({#3})}
\def\J_#1(#2){{\rm J}_#1\!\pr(#2)}
\def\cl{{\rm cl}\,}

\def\erfi{{\rm erfi}\,}

\def\half{{1 \over 2}}

\def\LL#1{L_#1}

\let\grad=\nabla
\let\lap=\Delta
\let\union=\bigcup

\def\ala{{\it \`a la\/}}
\def\apriori{{\it a priori\/}}
\def\apostiori{{\it a postiori\/}}


\def\fd#1{^{({#1})}}


\def\dx{\dkf{x}}
\def\dy{\dkf{y}}
\def\dz{\dkf{z}}
\def\dt{\dkf{t}}
\def\dV{\dkf{V}}
\def\ds{\dkf{\vc s}}

\def\ddxn^#1{{\dkf{}^#1 \over \dkfn^#1{x}}}

\def\ddx{{\dkf{} \over \dx}}
\def\pddx{{\partial \over \partial x}}
\def\pddy{{\partial \over \partial y}}

\def\pddxf#1{{\partial #1 \over \partial x}}
\def\pddyf#1{{\partial #1 \over \partial y}}

\def\Dv{{\cal D}}
\def\Dm{\Dv^{\vc m}}
\def\Dek{\Dv^{\vc{e}_k}}


\def\Bignorm#1{\Bigl\| #1 \Bigr\|}
\def\norm#1{\left\| #1 \right\|}
\def\Bignnnorm#1{ \Bigl | \mskip-1.5mu \Bigl\|\,{#1}\, \Bigr\|\mskip-1.5mu \Bigr |} 
\def\norminf#1{\norm{#1}_\infty}

\def\seq_#1^#2#3{\set{#3_{#1},\ldots,#3_{#2}}}
\def\infseq#1{\set{#1_{1},#1_{2},\ldots}}

\def\TT{\Bbb T}
\def\UU{\Bbb U}

\let\real=\R
\let\nonnegative=\N


\def\abs#1{\left|{#1}\right|}


\ffunction{f}
\ffunction{g}


%
%	Map a list using \mapfunction
%
% Usage:
% {\def \mapfunction#1{$#1^2$}
%
% \map a,b,c,d,\void.}


\def\mapengine#1,#2.{\mapfunction{#1}\ifx\void#2\else\mapengine #2.\fi }

\def\map[#1]{\mapengine #1,\void.}

\def\mapenginesep_#1#2,#3.{\mapfunction{#2}\ifx\void#3\else#1\mapengine #3.\fi }

\def\mapsep_#1[#2]{\mapenginesep_{#1}#2,\void.}

 \def\vczero{{\bf 0}}
 \def\vcone{{\bf 1}}
%\def\vcbr{\br}
\def\vcbr[#1]{\pr({#1})}


\def\bvect[#1,#2]{
{
\def\dots{\cdots}
\def\mapfunction##1{\ | \  ##1}
	\sopmatrix{
		 \,#1\map[#2]\,
	}
}
}

\def\vect[#1]{
{\def\dots{\ldots}
	\vcbr[{#1}]
}}

\def\vectt[#1]{
{\def\dots{\ldots}
	\vect[{#1}]^{\top}
}}

\def\Vectt[#1]{
{
\def\mapfunction##1{##1 \cr} 
\def\dots{\vdots}
	\sopmatrix{
		\map[#1]
	}
}}


\def\Notation#1{
\def\notationaddtab##1:##2={##1 & ##2\;& =}
\bigskip
\def\\{\cr\notationaddtab}
\halign{\quad\vtop{\parindent=0pt\hsize=0.33\hsize
						\strut##\strut}\hfil & \qquad \hfil $##$ & $##$ \hfil \cr\notationaddtab
	#1
}
\bigskip\noindent
}


\def\LHopital{L'Hopital's rule}

\def\qqquad{\qquad\quad}
\def\qqqquad{\qquad\qquad}

\def\qand{\quad\hbox{and}\quad}
\def\qqand{\qquad\hbox{and}\qquad}
\def\qfor{\quad\hbox{for}\quad}
\def\qqfor{\qquad\hbox{for}\qquad}
\def\qas{\quad\hbox{as}\quad}
\def\qqas{\qquad\hbox{as}\qquad}
\def\qqor{\qquad\hbox{or}\qquad}
\def\qqwhere{\qquad\hbox{where}\qquad}

\def\questionequals{= \!\!\!\!\!\!{\scriptstyle ? \atop }\,\,\,}
\def\simlimit_#1{\,\,\,\sim \!\!\!\!\!\!\!\!\!{ \atop \scriptscriptstyle #1 }}


\def\Xint#1{\mathchoice
   {\XXint\displaystyle\textstyle{#1}}%
   {\XXint\textstyle\scriptstyle{#1}}%
   {\XXint\scriptstyle\scriptscriptstyle{#1}}%
   {\XXint\scriptscriptstyle\scriptscriptstyle{#1}}%
   \!\int}
\def\XXint#1#2#3{{\setbox0=\hbox{$#1{#2#3}{\int}$}
     \vcenter{\hbox{$#2#3$}}\kern-.5\wd0}}
\def\ddashint{\Xint=}
\def\dashint{\Xint-}



\def\rad^#1#2{\,\,{}^#1\!\!\!\!\sqrt{#2}\,}




\def\Figuretwofixed#1#2#3\par{
\Figuretwow{#1}{#2}{0.48 \hsize}{#3}\par
}


\def\Painleve{Painlev\'e}

